SynStitch: a Self-Supervised Learning Network for Ultrasound Image Stitching Using Synthetic Training Pairs and Indirect Supervision

Ultrasound (US) image stitching can expand the field-of-view (FOV) by combining multiple US images from varied probe positions. However, registering US images with only partially overlapping anatomical contents is a challenging task. In this work, we introduce SynStitch, a self-supervised framework designed for 2DUS stitching. SynStitch consists of a synthetic stitching pair generation module (SSPGM) and an image stitching module (ISM). SSPGM utilizes a patch-conditioned ControlNet to generate realistic 2DUS stitching pairs with known affine matrix from a single input image. ISM then utilizes this synthetic paired data to learn 2DUS stitching in a supervised manner. Our framework was evaluated against multiple leading methods on a kidney ultrasound dataset, demonstrating superior 2DUS stitching performance through both qualitative and quantitative analyses. The code will be made public upon acceptance of the paper.

==> commentedOutFiguresEtc.tex <==
% \begin{figure*}
% \centering
% \includegraphics[width=1\textwidth]{./figure/stitch_results.pdf}
% \caption{\footnotesize Stitching results for samples from 5 subjects. From left to right: the first two columns, tagged in blue, display the source and target images for stitching. The third and fourth columns, tagged in yellow, show results from GlobalNet: the left column presents the overlay of the aligned source and fixed images, while the right column depicts the difference between the aligned source image and ground truth. Green contours outline the predicted aligned images, and red contours delineate the target and ground truth images. The fifth and sixth columns, tagged in pink, feature results from SynStitch, utilizing GlobalNet as the Image Stitching Module (ISM).}
% \label{stitch_results}
% \end{figure*}

% \begin{table*}
% \centering
% \caption{Quantitative Comparison of Stitching Performance}
% \label{table_test1}
% \begin{small} % Reduce font size
% \begin{tblr}{
%   colspec={|l|c|c|c|c|c|c|c|},
%   rows={m},
%   hline{1,3,5,7,9}={solid},
%   vline{1-7}={solid},
%   colsep=1.5pt, % Reduce column separation
%   rowsep=0.5pt % Reduce row separation
% }
% \toprule
% Metrics & ANTs & SIFT+RANSC & GlobalNet(GBN) & VoxelMorph(VXM) & LightGlue(LG) & SynthStitch-GBN & SynthStitch-VXM \\
% \midrule
% MSE(x100)\(\downarrow\) & 2.89 \(\pm\) 1.64 & 3.03 \(\pm\) 2.75 & 2.81 \(\pm\) 1.63 & 2.73 \(\pm\) 1.60 & 2.82 \(\pm\) 1.68 & \textbf{1.54\(\pm\) 1.14} & 1.90 \(\pm\) 1.38 \\
% SSIM\(\uparrow\) & 0.61 \(\pm\) 0.09 & 0.62 \(\pm\) 0.12 & 0.62 \(\pm\) 0.10 & 0.63 \(\pm\) 0.10 & 0.62 \(\pm\) 0.10 & \textbf{0.71 \(\pm\) 0.11} & 0.69 \(\pm\) 0.12 \\
% NCC\(\uparrow\) & 0.67 \(\pm\) 0.17 & 0.67 \(\pm\) 0.21 & 0.68 \(\pm\) 0.17 & 0.69 \(\pm\) 0.17 & 0.68 \(\pm\) 0.18 & \textbf{0.82 \(\pm\) 0.13} & 0.78 \(\pm\) 0.15 \\
% RMSE\(\downarrow\) & 5.13 \(\pm\) 2.63 & 4.93 \(\pm\) 3.35 & 5.21 \(\pm\) 2.62 & 5.01 \(\pm\) 2.62 & 5.09 \(\pm\) 2.67 & \textbf{3.36 \(\pm\) 1.94} & 3.75 \(\pm\) 2.20 \\
% \bottomrule
% \end{tblr}
% \end{small}
% \end{table*}

% \begin{table*}
% \centering
% \caption{Quantitative Comparison of 2DUS Stitching. \textbf{Bold} and \underline{underline} denote frameworks with best and second best performance for each metrics, respectively.}
% \label{table_test1}
% \begin{small} % Reduce font size
% \begin{tblr}{
%   colspec={|l|c|c|c|c|c|c|c|},
%   rows={m},
%   % hline{1,3,5,7,9}={solid},
%   hline{1,2,3,4,5}={solid},
%   vline{2-6}={solid},
%   colsep=1.5pt, % Reduce column separation
%   rowsep=0.5pt % Reduce row separation
% }
% \toprule
% Metrics & ANTs & SIFT+RANSC & GlobalNet & VoxelMorph & LightGlue & SynthStitch-VXM & SynthStitch-GLN \\
% \midrule
% MSE(x100)\(\downarrow\) & 2.89 \(\pm\) 1.64 & 3.03 \(\pm\) 2.75 & 2.81 \(\pm\) 1.63 & 2.73 \(\pm\) 1.60 & 2.82 \(\pm\) 1.68 & \underline{1.90 \(\pm\) 1.38} & \textbf{1.54\(\pm\) 1.14} \\
% SSIM\(\uparrow\) & 0.61 \(\pm\) 0.09 & 0.62 \(\pm\) 0.12 & 0.62 \(\pm\) 0.10 & 0.63 \(\pm\) 0.10 & 0.62 \(\pm\) 0.10 & \underline{0.69 \(\pm\) 0.12} & \textbf{0.71 \(\pm\) 0.11}\\
% NCC\(\uparrow\) & 0.67 \(\pm\) 0.17 & 0.67 \(\pm\) 0.21 & 0.68 \(\pm\) 0.17 & 0.69 \(\pm\) 0.17 & 0.68 \(\pm\) 0.18 & \underline{0.78 \(\pm\) 0.15} & \textbf{0.82 \(\pm\) 0.13}\\
% RMSE\(\downarrow\) & 5.13 \(\pm\) 2.63 & 4.93 \(\pm\) 3.35 & 5.21 \(\pm\) 2.62 & 5.01 \(\pm\) 2.62 & 5.09 \(\pm\) 2.67 & \underline{3.75 \(\pm\) 2.20}  & \textbf{3.36 \(\pm\) 1.94}\\
% \bottomrule
% \end{tblr}
% \end{small}
% \end{table*}

% \begin{table}[!t]
% \centering
% \caption{Quantitative Comparison of stitching performance}
% \label{table_test1}
% \begin{small} % Reduce font size
% \begin{tblr}{
%   colspec={|Q[l]|Q[c]|Q[c]|Q[c]|Q[c]|},
%   rows={m,0.05cm},
%   cell{1}{1}={r=2,c=1}{l},
%   cell{1}{2}={c=4}{c},
%   hline{1,2,3,5,8}={solid},
%   vline{1-4}={solid}, % Ensure only four columns
%   colsep=1pt, % Reduce column separation
%   rowsep=0.5pt % Reduce row separation
% }
% \toprule
% Methods & Metrics &  &  &  \\
% \cmidrule(lr{-1}){2-5}
% & {MSE(x100)\(\downarrow\)} & {SSIM\(\uparrow\)} & {NCC\(\uparrow\)} & {RMSE\(\downarrow\)}\\
% \midrule
% ANTs & 2.89 \(\pm\) 1.64 & 0.61  \(\pm\) 0.09& 0.67 \(\pm\) 0.17 & 5.13 \(\pm\)2.63 \\
% SIFT+RANSC & 3.03 \(\pm\) 2.75 & 0.62  \(\pm\) 0.12& 0.67 \(\pm\) 0.21 & 4.93 \(\pm\)3.35 \\
% GBN & 2.81 \(\pm\) 1.63 & 0.62 \(\pm\) 0.10& 0.68  \(\pm\) 0.17 & 5.21  \(\pm\)2.62 \\
% VXM & 2.73 \(\pm\) 1.60 & 0.63  \(\pm\) 0.10& 0.69 \(\pm\) 0.17 & 5.01 \(\pm\)2.62 \\
% LG & 2.82 \(\pm\) 1.68 &0.62 \(\pm\) 0.10& 0.68 \(\pm\) 0.18 & 5.09 \(\pm\) 2.67 \\
% SynthStitch(GBN) & \textbf{1.54\(\pm\) 1.14} & \textbf{0.71  \(\pm\) 0.11}& \textbf{0.82  \(\pm\) 0.13} & \textbf{3.36 \(\pm\)1.94} \\
% SynthStitch(VXM)& 1.90 \(\pm\) 1.38 & 0.69 \(\pm\) 0.12& 0.78 \(\pm\) 0.15 & 3.75 \(\pm\)2.20 \\
% % SynthStitch(LG)& - & -  \(\pm\) -& - \(\pm\) - & - \(\pm\)- \\

% \bottomrule
% \end{tblr}
% \end{small} % End of smaller font size
% \end{table}


% \begin{figure*}
% \centering
% \includegraphics[width=1\textwidth]{./figure/stitch_results.pdf}
% \caption{\footnotesize Stitching results for samples from 5 subjects. From left to right: the first two columns, tagged in blue, display the source and target images for stitching. The third and fourth columns, tagged in yellow, show results from GlobalNet: the left column presents the overlay of the aligned source and fixed images, while the right column depicts the difference between the aligned source image and ground truth. Green contours outline the predicted aligned images, and red contours delineate the target and ground truth images. The fifth and sixth columns, tagged in pink, feature results from SynStitch, utilizing GlobalNet as the Image Stitching Module (ISM).}
% \label{stitch_results}
% \end{figure*}

% \begin{figure}[!t]
% \centering
% \includegraphics[width=0.5\textwidth]{./figure/syn_examples.png}
% \caption{\footnotesize (a)Examples from the SynStitch Dataset. From left to right: original real ultrasound (US) image, affined real US image, and synthetic image generated by the pretrained SSPGM. The red contour highlights the condition used during generation. (b) 2-dimension embedding t-SNE of SynStitch Dataset.}
% \label{syn_examples}
% \end{figure}
